Towards Optimal Beacon Placement for Range-Aided Localization

Range-based localization is ubiquitous: global navigation satellite systems (GNSS) power mobile phone-based navigation, and autonomous mobile robots can use range measurements from a variety of modalities including sonar, radar, and even WiFi signals. Many of these localization systems rely on fixed anchors or beacons with known positions acting as transmitters or receivers. In this work, we answer a fundamental question: given a set of positions we would like to localize, how should beacons be placed so as to minimize localization error? Specifically, we present an information theoretic method for optimally selecting an arrangement consisting of a few beacons from a large set of candidate positions. By formulating localization as maximum a posteriori (MAP) estimation, we can cast beacon arrangement as a submodular set function maximization problem. This approach is probabilistically rigorous, simple to implement, and extremely flexible. Furthermore, we prove that the submodular structure of our problem formulation ensures that a greedy algorithm for beacon arrangement has suboptimality guarantees. We compare our method with a number of benchmarks on simulated data and release an open source Python implementation of our algorithm and experiments.

==> 2024-sequeira-optimal-beacon-crv-main-arxiv/2024-sequeira-optimal-beacon-crv-main/notation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Basic shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Matrices, vectors and linear algebra
\NewDocumentCommand\bbm{}{ \begin{bmatrix} }
\NewDocumentCommand\ebm{}{ \end{bmatrix} }
\NewDocumentCommand\Vector{m}{ \boldsymbol{\mathbf{#1}} }
\NewDocumentCommand\HomogeneousVector{m}{ \boldsymbol{#1} }
\NewDocumentCommand\Matrix{m}{ \boldsymbol{\mathbf{#1}} }
\NewDocumentCommand\Transpose{m}{ \left.{#1}\right.^\top }
\NewDocumentCommand\ConjugateTranspose{m}{ \left.{#1}\right.^H }
\NewDocumentCommand\PseudoInverse{m}{ #1^\dagger }
\NewDocumentCommand\Trace{m}{ \mathrm{tr}\left(#1\right) }
\NewDocumentCommand\Determinant{m}{ \mathrm{det}\left(#1\right) }
\NewDocumentCommand\Norm{m}{\left\Vert#1\right\Vert }
\NewDocumentCommand\FrobeniusNorm{m}{\Norm{#1}_{\scriptscriptstyle \mathrm{F}}}
\NewDocumentCommand\Diag{m}{ \mathrm{diag} \left( #1 \right) }
\NewDocumentCommand\Vectorize{m}{ \mathrm{vec}\left(#1 \right) }
\NewDocumentCommand\AbsoluteValue{m}{ \left\vert#1\right\vert }
\NewDocumentCommand\Kronecker{}{ \otimes }
\NewDocumentCommand\SingularValue{}{ \sigma }

%% Calculus
\NewDocumentCommand\dd{}{ \mathop{}\!\mathrm{d} }
\NewDocumentCommand\PartialDerivative{mm}{ \frac{\partial #1}{\partial #2} }
\NewDocumentCommand\OrdinaryDerivative{mm}{ \frac{\dd #1}{\dd #2} }
\NewDocumentCommand\Exp{m}{ \exp\left(#1\right) }
\NewDocumentCommand\Gradient{}{ \nabla }

%% Sets
\NewDocumentCommand\Set{m}{ \left\{#1\right\} }
\NewDocumentCommand\Real{}{ \mathbb{R} }
\NewDocumentCommand\Cardinality{m}{ \left\vert#1\right\vert }
\NewDocumentCommand\NonNegativeReal{}{ \Real_+ }
\NewDocumentCommand\Natural{}{ \mathbb{N} }
\NewDocumentCommand\Complex{}{ \mathbb{C} }
\NewDocumentCommand\Sym{m}{ \mathbb{S}^{#1} }
\NewDocumentCommand\PSD{m}{ \mathbb{S}^{#1}_+ }
\NewDocumentCommand\PD{m}{ \mathbb{S}^{#1}_{++} }
\NewDocumentCommand\Domain{m}{ \mathrm{dom}\left(#1\right) }
\NewDocumentCommand\Epigraph{m}{ \mathrm{epi}\left(#1\right) }
\NewDocumentCommand\Indices{m}{[#1]}
\NewDocumentCommand\Sphere{m}{\mathcal{S}^{#1}}
\NewDocumentCommand\HyperTorus{m}{\mathcal{T}^{#1}}
\NewDocumentCommand\Partition{}{ \mathcal{P} }

%% Lie groups and Lie algebras
\NewDocumentCommand\LieGroupSO{m}{ \mathrm{SO}(#1) }
\NewDocumentCommand\LieGroupO{m}{ \mathrm{O}(#1) }
\NewDocumentCommand\LieAlgebraSO{m}{ \mathfrak{so}(#1) }
\NewDocumentCommand\LieGroupSE{m}{ \mathrm{SE}(#1) }
\NewDocumentCommand\LieAlgebraSE{m}{ \mathfrak{se}(#1) }
\NewDocumentCommand\LieGroupSim{m}{ \mathrm{Sim}(#1) }
\NewDocumentCommand\LieAlgebraSim{m}{ \mathfrak{sim}(#1) }
\NewDocumentCommand\LieGroupAdjoint{m}{ \mathrm{Ad}\left(#1\right) }
\NewDocumentCommand\LieAlgebraAdjoint{m}{ \mathrm{ad}\left(#1\right) }
\NewDocumentCommand\LeftJacobianSE{}{ \Matrix{\mathcal{J}} }
\NewDocumentCommand\LeftJacobianSO{}{ \Matrix{J} }
\NewDocumentCommand\Wedge{m}{\left(#1\right)^\wedge}
\NewDocumentCommand\Vee{m}{\left(#1\right)^\wedge}

\NewDocumentCommand\MatLog{m}{\mathrm{Log}\left({#1}\right)}
\NewDocumentCommand\Matlog{m}{\mathrm{log}\Vee{#1}}
\NewDocumentCommand\MatExp{m}{\mathrm{Exp}\left({#1}\right)}
\NewDocumentCommand\Matexp{m}{\mathrm{exp}\Wedge{#1}}


%% Statistics and stochastic processes
\NewDocumentCommand\Expectation{mm}{ \mathbb{E}_{#2}\left[#1\right] }
\NewDocumentCommand\NormalDistribution{mm}{ \mathcal{N}\left(#1,#2\right) }
\NewDocumentCommand\LangevinDistribution{mm}{ \mathrm{Lang}\left(#1, #2\right) }
\NewDocumentCommand\ModeMatrix{}{ \Matrix{R}_\mu }
\NewDocumentCommand\Concentration{}{ \kappa }
\NewDocumentCommand\GaussianProcess{mm}{ \mathcal{GP}\left(#1,#2\right) }
\NewDocumentCommand\Noisy{m}{ \tilde{#1} }
\NewDocumentCommand\Covariance{}{ \Matrix{\Sigma} }
\NewDocumentCommand\FIM{}{ \Matrix{\mathcal{I}} }

%% Zero and Identity matrices
\NewDocumentCommand\Zero{}{ \Matrix{0} }
\NewDocumentCommand\Ones{}{ \Vector{1} }
\NewDocumentCommand\Identity{}{ \Matrix{I} }

%% Coordinate frames and transformations
\NewDocumentCommand\CoordinateFrame{m}{ \underrightarrow{\Matrix{\mathcal{F}}}_{#1} }
\NewDocumentCommand\Rotation{}{ \Matrix{R} }
\NewDocumentCommand\Translation{}{ \Vector{p} }
\NewDocumentCommand\RotationVector{}{ \Vector{\phi} }
\NewDocumentCommand\Quaternion{}{ \Vector{q} }
\NewDocumentCommand\QuaternionSpace{}{ \mathbb{H} }
\NewDocumentCommand\DualQuaternion{}{ \Vector{d} }
\NewDocumentCommand\DualQuaternionSpace{}{ \mathcal{H} }
\NewDocumentCommand\Transform{}{ \Matrix{T} }
\NewDocumentCommand\TransformVector{}{ \Vector{\xi} }
\NewDocumentCommand\Dim{}{ d }
\NewDocumentCommand\Homogenize{m}{ \bbm #1 \\ 1 \ebm }

%% Variable decorators
\NewDocumentCommand\Estimate{m}{\hat{#1}}
\NewDocumentCommand\Prior{m}{\check{#1}}
\NewDocumentCommand\Mean{m}{\overline{#1}}
\NewDocumentCommand\Optimal{m}{{#1}^*}


\NewDocumentCommand\Inv{m}{{#1}^{-1}}
\NewDocumentCommand\Defined{}{\triangleq}
\NewDocumentCommand\Define{}{ \triangleq }
\NewDocumentCommand\T{}{\mathsf{T}}

%% ====================================================== %%
%% Optimization
\NewDocumentCommand\ArgMax{m}{ \operatorname*{argmax}_{#1} }
\NewDocumentCommand\ArgMin{m}{ \operatorname*{argmin}_{#1} }
\NewDocumentCommand\Jacobian{m}{D_{#1}}
\NewDocumentCommand\CostMatrix{}{ \Matrix{C} }
%\NewDocumentCommand\CostFunction{}{ c } % Overloaded for this paper
\NewDocumentCommand\EqualityConstraintMatrix{}{ \Matrix{B} }
\NewDocumentCommand\InequalityConstraintMatrix{}{ \Matrix{A} }
\NewDocumentCommand\EqualityFunction{}{ h }
\NewDocumentCommand\InequalityFunction{}{ g }
\NewDocumentCommand\ActiveConstraintFunction{}{ f }
\NewDocumentCommand\Homogenizer{}{ s }
\NewDocumentCommand\NumEquality{}{ m }
\NewDocumentCommand\NumInequality{}{ l }
\NewDocumentCommand\NumActive{}{ k }
\NewDocumentCommand\Lagrangian{m}{ \mathcal{L}\left(#1\right) }
\NewDocumentCommand\LagrangianHessian{}{\Matrix{\mathcal{Q}}}
\NewDocumentCommand\LagrangeMultipliers{mm}{ \Lambda_{#1}\left(#2\right) }
\NewDocumentCommand\ActiveMultipliers{}{ \Vector{\mu} }
\NewDocumentCommand\LagrangeMapping{}{ \mathcal{M} }
\NewDocumentCommand\DualFunction{}{ \mathsf{d} }
\NewDocumentCommand\LICQ{m}{ \mathrm{LICQ}\left(#1\right) }
\NewDocumentCommand\ACQ{mm}{ \mathrm{ACQ}_{#1}\left(#2\right) }
\NewDocumentCommand\ActiveConstraints{m}{ A\left(#1\right) }
\NewDocumentCommand\LinearOperator{m}{ \mathcal{#1} }
\NewDocumentCommand\Parameter{}{ \xi }
\NewDocumentCommand\ParameterSpace{}{ \Xi }
\NewDocumentCommand\Stable{m}{ \bar{#1} }
\NewDocumentCommand\Value{m}{ \mathrm{val}\left(#1\right) }
\NewDocumentCommand\PrimalDualPair{}{ \Vector{\eta} }

%% Graph Theory
\NewDocumentCommand\Graph{}{ \mathcal{G} }
\NewDocumentCommand\Vertices{}{ \mathcal{V} }
\NewDocumentCommand\Edges{}{ \mathcal{E} }
\NewDocumentCommand\Clique{}{ \mathcal{C} }

\NewDocumentCommand\EqualityEdges{}{ \Edges_{\textrm{eq}} }
\NewDocumentCommand\IncidenceMatrix{m}{ \Matrix{B}(#1) }
\NewDocumentCommand\JointVertices{}{ \Vertices_{\mathrm{j}} }
\NewDocumentCommand\JointEdges{}{ \Edges_{\mathrm{l}} }
\NewDocumentCommand\AnchorEdges{}{ \Edges_{\mathrm{w}} }
\NewDocumentCommand\PlaneVertices{}{ \Vertices_{\mathrm{p}} }
\NewDocumentCommand\LeavingEdges{m}{ \delta(#1)^{-} }
\NewDocumentCommand\EnteringEdges{m}{ \delta(#1)^{+} }
\NewDocumentCommand\IncidentEdges{m}{ \delta(#1) }
\NewDocumentCommand\Neighbourhood{}{ \nu }

\newlength{\minuslength}
\settowidth{\minuslength}{$-$}

%% Optimal Beacon Placement
\NewDocumentCommand\NumBeacons{}{ N }
\NewDocumentCommand\NumPositions{}{ M }
\NewDocumentCommand\Budget{}{ K }
\NewDocumentCommand\FreeSpace{}{ \Omega }
\NewDocumentCommand\BeaconSet{}{ \mathcal{S} }
\NewDocumentCommand\CostFunction{}{ f_{\mathrm{D}} }
\NewDocumentCommand\CostFunctionNMS{}{ f_{\mathrm{D}}^+ }




==> 2024-sequeira-optimal-beacon-crv-main-arxiv/2024-sequeira-optimal-beacon-crv-main/packages.tex <==
\usepackage{times}

%\pdfinfo{
%   /Author (Homer Simpson)
%   /Title  (Robots: Our new overlords)
%   /CreationDate (D:20101201120000)
%   /Subject (Robots)
%   /Keywords (Robots;Overlords)
%}

% Removed for IJRR template clash?
%\usepackage[numbers]{natbib}

\usepackage{multicol}

%\usepackage[bookmarks=true]{hyperref}

%Custom imports
\usepackage{xparse}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{graphicx}
\usepackage{url}
\usepackage{booktabs}
\usepackage[para]{threeparttable}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{placeins}
\renewcommand\theadalign{br}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}

% Removed for IJRR template clash?
%\usepackage{hyperref}
%\hypersetup{colorlinks,linkcolor={blue},citecolor={green},urlcolor={blue}}

\usepackage{amsthm}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage[colorlinks,bookmarksopen,bookmarksnumbered,citecolor=red,urlcolor=red]{hyperref}
\usepackage[capitalize]{cleveref}
\usepackage{xcolor}
\usepackage{framed}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{pgfplots}
\usepackage{adjustbox}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}
\usepackage{flushend}

\captionsetup{font=small}
\captionsetup[sub]{font=small}

%% \usepackage{algorithmicx}
%% \usepackage{algorithm}
%% \usepackage[noend]{algpseudocode}
%\SetKwInOut{Parameters}{Parameters}
%\newcommand\mycommfont[1]{#1}
%\SetKwComment{Comment}{$\triangleright$\ }{}
%\SetCommentSty{mycommfont}
%\newcommand*\Let[2]{\State #1 $\gets$ #2}
%% \algrenewcommand\algorithmicrequire{\textbf{Input:}}
%% \algrenewcommand\algorithmicensure{\textbf{Output:}}
%% \algnewcommand\algorithmicinput{\textbf{Input:}}
%% \algnewcommand\INPUT{\item[\algorithmicinput]}

% To get the pretty pseudocode environments
\usepackage{algorithm}
\usepackage{algpseudocode}
% To enable proper indenting when forcibly breaking lines in algorithmic environments
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][0]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax}
\makeatother

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}



\usepackage{setspace}
\usepackage[normalem]{ulem}

\colorlet{shadecolor}{gray!10}
\newenvironment{todo}[1]
   {\begin{shaded} {\color{red}\textbf{To-do}} (\textit{#1}).}
   {\end{shaded}}
\newtheorem{problem}{Problem}
%\crefname{problem}{Problem}{Problems}
\newtheorem{assumption}{Assumption}
%\crefname{assumption}{Assumption}{Assumptions}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
%\crefname{proposition}{Proposition}{Propositions}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}


==> 2024-sequeira-optimal-beacon-crv-main-arxiv__2_/notation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Basic shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Matrices, vectors and linear algebra
\NewDocumentCommand\bbm{}{ \begin{bmatrix} }
\NewDocumentCommand\ebm{}{ \end{bmatrix} }
\NewDocumentCommand\Vector{m}{ \boldsymbol{\mathbf{#1}} }
\NewDocumentCommand\HomogeneousVector{m}{ \boldsymbol{#1} }
\NewDocumentCommand\Matrix{m}{ \boldsymbol{\mathbf{#1}} }
\NewDocumentCommand\Transpose{m}{ \left.{#1}\right.^\top }
\NewDocumentCommand\ConjugateTranspose{m}{ \left.{#1}\right.^H }
\NewDocumentCommand\PseudoInverse{m}{ #1^\dagger }
\NewDocumentCommand\Trace{m}{ \mathrm{tr}\left(#1\right) }
\NewDocumentCommand\Determinant{m}{ \mathrm{det}\left(#1\right) }
\NewDocumentCommand\Norm{m}{\left\Vert#1\right\Vert }
\NewDocumentCommand\FrobeniusNorm{m}{\Norm{#1}_{\scriptscriptstyle \mathrm{F}}}
\NewDocumentCommand\Diag{m}{ \mathrm{diag} \left( #1 \right) }
\NewDocumentCommand\Vectorize{m}{ \mathrm{vec}\left(#1 \right) }
\NewDocumentCommand\AbsoluteValue{m}{ \left\vert#1\right\vert }
\NewDocumentCommand\Kronecker{}{ \otimes }
\NewDocumentCommand\SingularValue{}{ \sigma }

%% Calculus
\NewDocumentCommand\dd{}{ \mathop{}\!\mathrm{d} }
\NewDocumentCommand\PartialDerivative{mm}{ \frac{\partial #1}{\partial #2} }
\NewDocumentCommand\OrdinaryDerivative{mm}{ \frac{\dd #1}{\dd #2} }
\NewDocumentCommand\Exp{m}{ \exp\left(#1\right) }
\NewDocumentCommand\Gradient{}{ \nabla }

%% Sets
\NewDocumentCommand\Set{m}{ \left\{#1\right\} }
\NewDocumentCommand\Real{}{ \mathbb{R} }
\NewDocumentCommand\Cardinality{m}{ \left\vert#1\right\vert }
\NewDocumentCommand\NonNegativeReal{}{ \Real_+ }
\NewDocumentCommand\Natural{}{ \mathbb{N} }
\NewDocumentCommand\Complex{}{ \mathbb{C} }
\NewDocumentCommand\Sym{m}{ \mathbb{S}^{#1} }
\NewDocumentCommand\PSD{m}{ \mathbb{S}^{#1}_+ }
\NewDocumentCommand\PD{m}{ \mathbb{S}^{#1}_{++} }
\NewDocumentCommand\Domain{m}{ \mathrm{dom}\left(#1\right) }
\NewDocumentCommand\Epigraph{m}{ \mathrm{epi}\left(#1\right) }
\NewDocumentCommand\Indices{m}{[#1]}
\NewDocumentCommand\Sphere{m}{\mathcal{S}^{#1}}
\NewDocumentCommand\HyperTorus{m}{\mathcal{T}^{#1}}
\NewDocumentCommand\Partition{}{ \mathcal{P} }

%% Lie groups and Lie algebras
\NewDocumentCommand\LieGroupSO{m}{ \mathrm{SO}(#1) }
\NewDocumentCommand\LieGroupO{m}{ \mathrm{O}(#1) }
\NewDocumentCommand\LieAlgebraSO{m}{ \mathfrak{so}(#1) }
\NewDocumentCommand\LieGroupSE{m}{ \mathrm{SE}(#1) }
\NewDocumentCommand\LieAlgebraSE{m}{ \mathfrak{se}(#1) }
\NewDocumentCommand\LieGroupSim{m}{ \mathrm{Sim}(#1) }
\NewDocumentCommand\LieAlgebraSim{m}{ \mathfrak{sim}(#1) }
\NewDocumentCommand\LieGroupAdjoint{m}{ \mathrm{Ad}\left(#1\right) }
\NewDocumentCommand\LieAlgebraAdjoint{m}{ \mathrm{ad}\left(#1\right) }
\NewDocumentCommand\LeftJacobianSE{}{ \Matrix{\mathcal{J}} }
\NewDocumentCommand\LeftJacobianSO{}{ \Matrix{J} }
\NewDocumentCommand\Wedge{m}{\left(#1\right)^\wedge}
\NewDocumentCommand\Vee{m}{\left(#1\right)^\wedge}

\NewDocumentCommand\MatLog{m}{\mathrm{Log}\left({#1}\right)}
\NewDocumentCommand\Matlog{m}{\mathrm{log}\Vee{#1}}
\NewDocumentCommand\MatExp{m}{\mathrm{Exp}\left({#1}\right)}
\NewDocumentCommand\Matexp{m}{\mathrm{exp}\Wedge{#1}}


%% Statistics and stochastic processes
\NewDocumentCommand\Expectation{mm}{ \mathbb{E}_{#2}\left[#1\right] }
\NewDocumentCommand\NormalDistribution{mm}{ \mathcal{N}\left(#1,#2\right) }
\NewDocumentCommand\LangevinDistribution{mm}{ \mathrm{Lang}\left(#1, #2\right) }
\NewDocumentCommand\ModeMatrix{}{ \Matrix{R}_\mu }
\NewDocumentCommand\Concentration{}{ \kappa }
\NewDocumentCommand\GaussianProcess{mm}{ \mathcal{GP}\left(#1,#2\right) }
\NewDocumentCommand\Noisy{m}{ \tilde{#1} }
\NewDocumentCommand\Covariance{}{ \Matrix{\Sigma} }
\NewDocumentCommand\FIM{}{ \Matrix{\mathcal{I}} }

%% Zero and Identity matrices
\NewDocumentCommand\Zero{}{ \Matrix{0} }
\NewDocumentCommand\Ones{}{ \Vector{1} }
\NewDocumentCommand\Identity{}{ \Matrix{I} }

%% Coordinate frames and transformations
\NewDocumentCommand\CoordinateFrame{m}{ \underrightarrow{\Matrix{\mathcal{F}}}_{#1} }
\NewDocumentCommand\Rotation{}{ \Matrix{R} }
\NewDocumentCommand\Translation{}{ \Vector{p} }
\NewDocumentCommand\RotationVector{}{ \Vector{\phi} }
\NewDocumentCommand\Quaternion{}{ \Vector{q} }
\NewDocumentCommand\QuaternionSpace{}{ \mathbb{H} }
\NewDocumentCommand\DualQuaternion{}{ \Vector{d} }
\NewDocumentCommand\DualQuaternionSpace{}{ \mathcal{H} }
\NewDocumentCommand\Transform{}{ \Matrix{T} }
\NewDocumentCommand\TransformVector{}{ \Vector{\xi} }
\NewDocumentCommand\Dim{}{ d }
\NewDocumentCommand\Homogenize{m}{ \bbm #1 \\ 1 \ebm }

%% Variable decorators
\NewDocumentCommand\Estimate{m}{\hat{#1}}
\NewDocumentCommand\Prior{m}{\check{#1}}
\NewDocumentCommand\Mean{m}{\overline{#1}}
\NewDocumentCommand\Optimal{m}{{#1}^*}


\NewDocumentCommand\Inv{m}{{#1}^{-1}}
\NewDocumentCommand\Defined{}{\triangleq}
\NewDocumentCommand\Define{}{ \triangleq }
\NewDocumentCommand\T{}{\mathsf{T}}

%% ====================================================== %%
%% Optimization
\NewDocumentCommand\ArgMax{m}{ \operatorname*{argmax}_{#1} }
\NewDocumentCommand\ArgMin{m}{ \operatorname*{argmin}_{#1} }
\NewDocumentCommand\Jacobian{m}{D_{#1}}
\NewDocumentCommand\CostMatrix{}{ \Matrix{C} }
%\NewDocumentCommand\CostFunction{}{ c } % Overloaded for this paper
\NewDocumentCommand\EqualityConstraintMatrix{}{ \Matrix{B} }
\NewDocumentCommand\InequalityConstraintMatrix{}{ \Matrix{A} }
\NewDocumentCommand\EqualityFunction{}{ h }
\NewDocumentCommand\InequalityFunction{}{ g }
\NewDocumentCommand\ActiveConstraintFunction{}{ f }
\NewDocumentCommand\Homogenizer{}{ s }
\NewDocumentCommand\NumEquality{}{ m }
\NewDocumentCommand\NumInequality{}{ l }
\NewDocumentCommand\NumActive{}{ k }
\NewDocumentCommand\Lagrangian{m}{ \mathcal{L}\left(#1\right) }
\NewDocumentCommand\LagrangianHessian{}{\Matrix{\mathcal{Q}}}
\NewDocumentCommand\LagrangeMultipliers{mm}{ \Lambda_{#1}\left(#2\right) }
\NewDocumentCommand\ActiveMultipliers{}{ \Vector{\mu} }
\NewDocumentCommand\LagrangeMapping{}{ \mathcal{M} }
\NewDocumentCommand\DualFunction{}{ \mathsf{d} }
\NewDocumentCommand\LICQ{m}{ \mathrm{LICQ}\left(#1\right) }
\NewDocumentCommand\ACQ{mm}{ \mathrm{ACQ}_{#1}\left(#2\right) }
\NewDocumentCommand\ActiveConstraints{m}{ A\left(#1\right) }
\NewDocumentCommand\LinearOperator{m}{ \mathcal{#1} }
\NewDocumentCommand\Parameter{}{ \xi }
\NewDocumentCommand\ParameterSpace{}{ \Xi }
\NewDocumentCommand\Stable{m}{ \bar{#1} }
\NewDocumentCommand\Value{m}{ \mathrm{val}\left(#1\right) }
\NewDocumentCommand\PrimalDualPair{}{ \Vector{\eta} }

%% Graph Theory
\NewDocumentCommand\Graph{}{ \mathcal{G} }
\NewDocumentCommand\Vertices{}{ \mathcal{V} }
\NewDocumentCommand\Edges{}{ \mathcal{E} }
\NewDocumentCommand\Clique{}{ \mathcal{C} }

\NewDocumentCommand\EqualityEdges{}{ \Edges_{\textrm{eq}} }
\NewDocumentCommand\IncidenceMatrix{m}{ \Matrix{B}(#1) }
\NewDocumentCommand\JointVertices{}{ \Vertices_{\mathrm{j}} }
\NewDocumentCommand\JointEdges{}{ \Edges_{\mathrm{l}} }
\NewDocumentCommand\AnchorEdges{}{ \Edges_{\mathrm{w}} }
\NewDocumentCommand\PlaneVertices{}{ \Vertices_{\mathrm{p}} }
\NewDocumentCommand\LeavingEdges{m}{ \delta(#1)^{-} }
\NewDocumentCommand\EnteringEdges{m}{ \delta(#1)^{+} }
\NewDocumentCommand\IncidentEdges{m}{ \delta(#1) }
\NewDocumentCommand\Neighbourhood{}{ \nu }

\newlength{\minuslength}
\settowidth{\minuslength}{$-$}

%% Optimal Beacon Placement
\NewDocumentCommand\NumBeacons{}{ N }
\NewDocumentCommand\NumPositions{}{ M }
\NewDocumentCommand\Budget{}{ K }
\NewDocumentCommand\FreeSpace{}{ \Omega }
\NewDocumentCommand\BeaconSet{}{ \mathcal{S} }
\NewDocumentCommand\CostFunction{}{ f_{\mathrm{D}} }
\NewDocumentCommand\CostFunctionNMS{}{ f_{\mathrm{D}}^+ }




==> 2024-sequeira-optimal-beacon-crv-main-arxiv__2_/packages.tex <==
\usepackage{times}

%\pdfinfo{
%   /Author (Homer Simpson)
%   /Title  (Robots: Our new overlords)
%   /CreationDate (D:20101201120000)
%   /Subject (Robots)
%   /Keywords (Robots;Overlords)
%}

% Removed for IJRR template clash?
%\usepackage[numbers]{natbib}

\usepackage{multicol}

%\usepackage[bookmarks=true]{hyperref}

%Custom imports
\usepackage{xparse}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{graphicx}
\usepackage{url}
\usepackage{booktabs}
\usepackage[para]{threeparttable}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{placeins}
\renewcommand\theadalign{br}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}

% Removed for IJRR template clash?
%\usepackage{hyperref}
%\hypersetup{colorlinks,linkcolor={blue},citecolor={green},urlcolor={blue}}

\usepackage{amsthm}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage[colorlinks,bookmarksopen,bookmarksnumbered,citecolor=red,urlcolor=red]{hyperref}
\usepackage[capitalize]{cleveref}
\usepackage{xcolor}
\usepackage{framed}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{pgfplots}
\usepackage{adjustbox}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}
\usepackage{flushend}

\captionsetup{font=small}
\captionsetup[sub]{font=small}

%% \usepackage{algorithmicx}
%% \usepackage{algorithm}
%% \usepackage[noend]{algpseudocode}
%\SetKwInOut{Parameters}{Parameters}
%\newcommand\mycommfont[1]{#1}
%\SetKwComment{Comment}{$\triangleright$\ }{}
%\SetCommentSty{mycommfont}
%\newcommand*\Let[2]{\State #1 $\gets$ #2}
%% \algrenewcommand\algorithmicrequire{\textbf{Input:}}
%% \algrenewcommand\algorithmicensure{\textbf{Output:}}
%% \algnewcommand\algorithmicinput{\textbf{Input:}}
%% \algnewcommand\INPUT{\item[\algorithmicinput]}

% To get the pretty pseudocode environments
\usepackage{algorithm}
\usepackage{algpseudocode}
% To enable proper indenting when forcibly breaking lines in algorithmic environments
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][0]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax}
\makeatother

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}



\usepackage{setspace}
\usepackage[normalem]{ulem}

\colorlet{shadecolor}{gray!10}
\newenvironment{todo}[1]
   {\begin{shaded} {\color{red}\textbf{To-do}} (\textit{#1}).}
   {\end{shaded}}
\newtheorem{problem}{Problem}
%\crefname{problem}{Problem}{Problems}
\newtheorem{assumption}{Assumption}
%\crefname{assumption}{Assumption}{Assumptions}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
%\crefname{proposition}{Proposition}{Propositions}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}


==> 2024-sequeira-optimal-beacon-crv-main/notation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Basic shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Matrices, vectors and linear algebra
\NewDocumentCommand\bbm{}{ \begin{bmatrix} }
\NewDocumentCommand\ebm{}{ \end{bmatrix} }
\NewDocumentCommand\Vector{m}{ \boldsymbol{\mathbf{#1}} }
\NewDocumentCommand\HomogeneousVector{m}{ \boldsymbol{#1} }
\NewDocumentCommand\Matrix{m}{ \boldsymbol{\mathbf{#1}} }
\NewDocumentCommand\Transpose{m}{ \left.{#1}\right.^\top }
\NewDocumentCommand\ConjugateTranspose{m}{ \left.{#1}\right.^H }
\NewDocumentCommand\PseudoInverse{m}{ #1^\dagger }
\NewDocumentCommand\Trace{m}{ \mathrm{tr}\left(#1\right) }
\NewDocumentCommand\Determinant{m}{ \mathrm{det}\left(#1\right) }
\NewDocumentCommand\Norm{m}{\left\Vert#1\right\Vert }
\NewDocumentCommand\FrobeniusNorm{m}{\Norm{#1}_{\scriptscriptstyle \mathrm{F}}}
\NewDocumentCommand\Diag{m}{ \mathrm{diag} \left( #1 \right) }
\NewDocumentCommand\Vectorize{m}{ \mathrm{vec}\left(#1 \right) }
\NewDocumentCommand\AbsoluteValue{m}{ \left\vert#1\right\vert }
\NewDocumentCommand\Kronecker{}{ \otimes }
\NewDocumentCommand\SingularValue{}{ \sigma }

%% Calculus
\NewDocumentCommand\dd{}{ \mathop{}\!\mathrm{d} }
\NewDocumentCommand\PartialDerivative{mm}{ \frac{\partial #1}{\partial #2} }
\NewDocumentCommand\OrdinaryDerivative{mm}{ \frac{\dd #1}{\dd #2} }
\NewDocumentCommand\Exp{m}{ \exp\left(#1\right) }
\NewDocumentCommand\Gradient{}{ \nabla }

%% Sets
\NewDocumentCommand\Set{m}{ \left\{#1\right\} }
\NewDocumentCommand\Real{}{ \mathbb{R} }
\NewDocumentCommand\Cardinality{m}{ \left\vert#1\right\vert }
\NewDocumentCommand\NonNegativeReal{}{ \Real_+ }
\NewDocumentCommand\Natural{}{ \mathbb{N} }
\NewDocumentCommand\Complex{}{ \mathbb{C} }
\NewDocumentCommand\Sym{m}{ \mathbb{S}^{#1} }
\NewDocumentCommand\PSD{m}{ \mathbb{S}^{#1}_+ }
\NewDocumentCommand\PD{m}{ \mathbb{S}^{#1}_{++} }
\NewDocumentCommand\Domain{m}{ \mathrm{dom}\left(#1\right) }
\NewDocumentCommand\Epigraph{m}{ \mathrm{epi}\left(#1\right) }
\NewDocumentCommand\Indices{m}{[#1]}
\NewDocumentCommand\Sphere{m}{\mathcal{S}^{#1}}
\NewDocumentCommand\HyperTorus{m}{\mathcal{T}^{#1}}
\NewDocumentCommand\Partition{}{ \mathcal{P} }

%% Lie groups and Lie algebras
\NewDocumentCommand\LieGroupSO{m}{ \mathrm{SO}(#1) }
\NewDocumentCommand\LieGroupO{m}{ \mathrm{O}(#1) }
\NewDocumentCommand\LieAlgebraSO{m}{ \mathfrak{so}(#1) }
\NewDocumentCommand\LieGroupSE{m}{ \mathrm{SE}(#1) }
\NewDocumentCommand\LieAlgebraSE{m}{ \mathfrak{se}(#1) }
\NewDocumentCommand\LieGroupSim{m}{ \mathrm{Sim}(#1) }
\NewDocumentCommand\LieAlgebraSim{m}{ \mathfrak{sim}(#1) }
\NewDocumentCommand\LieGroupAdjoint{m}{ \mathrm{Ad}\left(#1\right) }
\NewDocumentCommand\LieAlgebraAdjoint{m}{ \mathrm{ad}\left(#1\right) }
\NewDocumentCommand\LeftJacobianSE{}{ \Matrix{\mathcal{J}} }
\NewDocumentCommand\LeftJacobianSO{}{ \Matrix{J} }
\NewDocumentCommand\Wedge{m}{\left(#1\right)^\wedge}
\NewDocumentCommand\Vee{m}{\left(#1\right)^\wedge}

\NewDocumentCommand\MatLog{m}{\mathrm{Log}\left({#1}\right)}
\NewDocumentCommand\Matlog{m}{\mathrm{log}\Vee{#1}}
\NewDocumentCommand\MatExp{m}{\mathrm{Exp}\left({#1}\right)}
\NewDocumentCommand\Matexp{m}{\mathrm{exp}\Wedge{#1}}


%% Statistics and stochastic processes
\NewDocumentCommand\Expectation{mm}{ \mathbb{E}_{#2}\left[#1\right] }
\NewDocumentCommand\NormalDistribution{mm}{ \mathcal{N}\left(#1,#2\right) }
\NewDocumentCommand\LangevinDistribution{mm}{ \mathrm{Lang}\left(#1, #2\right) }
\NewDocumentCommand\ModeMatrix{}{ \Matrix{R}_\mu }
\NewDocumentCommand\Concentration{}{ \kappa }
\NewDocumentCommand\GaussianProcess{mm}{ \mathcal{GP}\left(#1,#2\right) }
\NewDocumentCommand\Noisy{m}{ \tilde{#1} }
\NewDocumentCommand\Covariance{}{ \Matrix{\Sigma} }
\NewDocumentCommand\FIM{}{ \Matrix{\mathcal{I}} }

%% Zero and Identity matrices
\NewDocumentCommand\Zero{}{ \Matrix{0} }
\NewDocumentCommand\Ones{}{ \Vector{1} }
\NewDocumentCommand\Identity{}{ \Matrix{I} }

%% Coordinate frames and transformations
\NewDocumentCommand\CoordinateFrame{m}{ \underrightarrow{\Matrix{\mathcal{F}}}_{#1} }
\NewDocumentCommand\Rotation{}{ \Matrix{R} }
\NewDocumentCommand\Translation{}{ \Vector{p} }
\NewDocumentCommand\RotationVector{}{ \Vector{\phi} }
\NewDocumentCommand\Quaternion{}{ \Vector{q} }
\NewDocumentCommand\QuaternionSpace{}{ \mathbb{H} }
\NewDocumentCommand\DualQuaternion{}{ \Vector{d} }
\NewDocumentCommand\DualQuaternionSpace{}{ \mathcal{H} }
\NewDocumentCommand\Transform{}{ \Matrix{T} }
\NewDocumentCommand\TransformVector{}{ \Vector{\xi} }
\NewDocumentCommand\Dim{}{ d }
\NewDocumentCommand\Homogenize{m}{ \bbm #1 \\ 1 \ebm }

%% Variable decorators
\NewDocumentCommand\Estimate{m}{\hat{#1}}
\NewDocumentCommand\Prior{m}{\check{#1}}
\NewDocumentCommand\Mean{m}{\overline{#1}}
\NewDocumentCommand\Optimal{m}{{#1}^*}


\NewDocumentCommand\Inv{m}{{#1}^{-1}}
\NewDocumentCommand\Defined{}{\triangleq}
\NewDocumentCommand\Define{}{ \triangleq }
\NewDocumentCommand\T{}{\mathsf{T}}

%% ====================================================== %%
%% Optimization
\NewDocumentCommand\ArgMax{m}{ \operatorname*{argmax}_{#1} }
\NewDocumentCommand\ArgMin{m}{ \operatorname*{argmin}_{#1} }
\NewDocumentCommand\Jacobian{m}{D_{#1}}
\NewDocumentCommand\CostMatrix{}{ \Matrix{C} }
%\NewDocumentCommand\CostFunction{}{ c } % Overloaded for this paper
\NewDocumentCommand\EqualityConstraintMatrix{}{ \Matrix{B} }
\NewDocumentCommand\InequalityConstraintMatrix{}{ \Matrix{A} }
\NewDocumentCommand\EqualityFunction{}{ h }
\NewDocumentCommand\InequalityFunction{}{ g }
\NewDocumentCommand\ActiveConstraintFunction{}{ f }
\NewDocumentCommand\Homogenizer{}{ s }
\NewDocumentCommand\NumEquality{}{ m }
\NewDocumentCommand\NumInequality{}{ l }
\NewDocumentCommand\NumActive{}{ k }
\NewDocumentCommand\Lagrangian{m}{ \mathcal{L}\left(#1\right) }
\NewDocumentCommand\LagrangianHessian{}{\Matrix{\mathcal{Q}}}
\NewDocumentCommand\LagrangeMultipliers{mm}{ \Lambda_{#1}\left(#2\right) }
\NewDocumentCommand\ActiveMultipliers{}{ \Vector{\mu} }
\NewDocumentCommand\LagrangeMapping{}{ \mathcal{M} }
\NewDocumentCommand\DualFunction{}{ \mathsf{d} }
\NewDocumentCommand\LICQ{m}{ \mathrm{LICQ}\left(#1\right) }
\NewDocumentCommand\ACQ{mm}{ \mathrm{ACQ}_{#1}\left(#2\right) }
\NewDocumentCommand\ActiveConstraints{m}{ A\left(#1\right) }
\NewDocumentCommand\LinearOperator{m}{ \mathcal{#1} }
\NewDocumentCommand\Parameter{}{ \xi }
\NewDocumentCommand\ParameterSpace{}{ \Xi }
\NewDocumentCommand\Stable{m}{ \bar{#1} }
\NewDocumentCommand\Value{m}{ \mathrm{val}\left(#1\right) }
\NewDocumentCommand\PrimalDualPair{}{ \Vector{\eta} }

%% Graph Theory
\NewDocumentCommand\Graph{}{ \mathcal{G} }
\NewDocumentCommand\Vertices{}{ \mathcal{V} }
\NewDocumentCommand\Edges{}{ \mathcal{E} }
\NewDocumentCommand\Clique{}{ \mathcal{C} }

\NewDocumentCommand\EqualityEdges{}{ \Edges_{\textrm{eq}} }
\NewDocumentCommand\IncidenceMatrix{m}{ \Matrix{B}(#1) }
\NewDocumentCommand\JointVertices{}{ \Vertices_{\mathrm{j}} }
\NewDocumentCommand\JointEdges{}{ \Edges_{\mathrm{l}} }
\NewDocumentCommand\AnchorEdges{}{ \Edges_{\mathrm{w}} }
\NewDocumentCommand\PlaneVertices{}{ \Vertices_{\mathrm{p}} }
\NewDocumentCommand\LeavingEdges{m}{ \delta(#1)^{-} }
\NewDocumentCommand\EnteringEdges{m}{ \delta(#1)^{+} }
\NewDocumentCommand\IncidentEdges{m}{ \delta(#1) }
\NewDocumentCommand\Neighbourhood{}{ \nu }

\newlength{\minuslength}
\settowidth{\minuslength}{$-$}

%% Optimal Beacon Placement
\NewDocumentCommand\NumBeacons{}{ N }
\NewDocumentCommand\NumPositions{}{ M }
\NewDocumentCommand\Budget{}{ K }
\NewDocumentCommand\FreeSpace{}{ \Omega }
\NewDocumentCommand\BeaconSet{}{ \mathcal{S} }
\NewDocumentCommand\CostFunction{}{ f_{\mathrm{D}} }
\NewDocumentCommand\CostFunctionNMS{}{ f_{\mathrm{D}}^+ }




==> 2024-sequeira-optimal-beacon-crv-main/packages.tex <==
\usepackage{times}

%\pdfinfo{
%   /Author (Homer Simpson)
%   /Title  (Robots: Our new overlords)
%   /CreationDate (D:20101201120000)
%   /Subject (Robots)
%   /Keywords (Robots;Overlords)
%}

% Removed for IJRR template clash?
%\usepackage[numbers]{natbib}

\usepackage{multicol}

%\usepackage[bookmarks=true]{hyperref}

%Custom imports
\usepackage{xparse}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{graphicx}
\usepackage{url}
\usepackage{booktabs}
\usepackage[para]{threeparttable}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{placeins}
\renewcommand\theadalign{br}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}

% Removed for IJRR template clash?
%\usepackage{hyperref}
%\hypersetup{colorlinks,linkcolor={blue},citecolor={green},urlcolor={blue}}

\usepackage{amsthm}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage[colorlinks,bookmarksopen,bookmarksnumbered,citecolor=red,urlcolor=red]{hyperref}
\usepackage[capitalize]{cleveref}
\usepackage{xcolor}
\usepackage{framed}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{pgfplots}
\usepackage{adjustbox}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}
\usepackage{flushend}

\captionsetup{font=small}
\captionsetup[sub]{font=small}

%% \usepackage{algorithmicx}
%% \usepackage{algorithm}
%% \usepackage[noend]{algpseudocode}
%\SetKwInOut{Parameters}{Parameters}
%\newcommand\mycommfont[1]{#1}
%\SetKwComment{Comment}{$\triangleright$\ }{}
%\SetCommentSty{mycommfont}
%\newcommand*\Let[2]{\State #1 $\gets$ #2}
%% \algrenewcommand\algorithmicrequire{\textbf{Input:}}
%% \algrenewcommand\algorithmicensure{\textbf{Output:}}
%% \algnewcommand\algorithmicinput{\textbf{Input:}}
%% \algnewcommand\INPUT{\item[\algorithmicinput]}

% To get the pretty pseudocode environments
\usepackage{algorithm}
\usepackage{algpseudocode}
% To enable proper indenting when forcibly breaking lines in algorithmic environments
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][0]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax}
\makeatother

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}



\usepackage{setspace}
\usepackage[normalem]{ulem}

\colorlet{shadecolor}{gray!10}
\newenvironment{todo}[1]
   {\begin{shaded} {\color{red}\textbf{To-do}} (\textit{#1}).}
   {\end{shaded}}
\newtheorem{problem}{Problem}
%\crefname{problem}{Problem}{Problems}
\newtheorem{assumption}{Assumption}
%\crefname{assumption}{Assumption}{Assumptions}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
%\crefname{proposition}{Proposition}{Propositions}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}

